PSO-Convolutional Neural Networks with Heterogeneous Learning Rate

Convolutional Neural Networks (ConvNets or CNNs) have been candidly deployed in the scope of computer vision and related fields. Nevertheless, the dynamics of training of these neural networks lie still elusive: it is hard and computationally expensive to train them. A myriad of architectures and training strategies have been proposed to overcome this challenge and address several problems in image processing such as speech, image and action recognition as well as object detection. In this article, we propose a novel Particle Swarm Optimization (PSO) based training for ConvNets. In such framework, the vector of weights of each ConvNet is typically cast as the position of a particle in phase space whereby PSO collaborative dynamics intertwines with Stochastic Gradient Descent (SGD) in order to boost training performance and generalization. Our approach goes as follows: i) [regular phase] each ConvNet is trained independently via SGD; ii) [collaborative phase] ConvNets share among themselves their current vector of weights (or particle-position) along with their gradient estimates of the Loss function. Distinct step sizes are coined by distinct ConvNets. By properly blending ConvNets with large (possibly random) step-sizes along with more conservative ones, we propose an algorithm with competitive performance with respect to other PSO-based approaches on Cifar-10 and Cifar-100 (accuracy of 98.31% and 87.48%). These accuracy levels are obtained by resorting to only four ConvNets -- such results are expected to scale with the number of collaborative ConvNets accordingly. We make our source codes available for download https://github.com/leonlha/PSO-ConvNet-Dynamics.

==> table_adv_experiments2.tex <==
% \usepackage{color}


\begin{table*}
\centering
\caption{}
\label{tab:gradients2}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|} 
\hline
\multicolumn{15}{|c|}{\begin{tabular}[c]{@{}c@{}}\\\\Parameters\end{tabular}}                                                                                                                                                                                                                                                                                                                                      & \multicolumn{4}{c|}{Accuracy}                                                                                                                                                      \\ 
\cline{1-15}
\multicolumn{2}{|c|}{KNN}                        & \multicolumn{1}{c|}{Warmup} & \multicolumn{12}{c|}{Gradient}                                                                                                                                                                                                                                                                                                    & \multicolumn{4}{c|}{}                                                                                                                                                              \\ 
\cline{1-2}\cline{4-19}
\multicolumn{1}{|c|}{k} & \multicolumn{1}{c|}{C} & \multicolumn{1}{c|}{}       & \multicolumn{3}{c|}{PSO-1}                                                     & \multicolumn{3}{c|}{PSO-2}                                                     & \multicolumn{3}{c|}{PSO-3}                                                     & \multicolumn{3}{c|}{PSO-4}                                                     & \multicolumn{1}{c}{PSO-1}                  & \multicolumn{1}{c}{PSO-2}                  & \multicolumn{1}{c}{PSO-3}                  & PSO-4                                       \\ 
\cline{4-15}
\multicolumn{1}{|c|}{}  & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{}       & \multicolumn{1}{c|}{M12} & \multicolumn{1}{c|}{M13} & \multicolumn{1}{c|}{M14} & \multicolumn{1}{c|}{M21} & \multicolumn{1}{c|}{M23} & \multicolumn{1}{c|}{M24} & \multicolumn{1}{c|}{M31} & \multicolumn{1}{c|}{M32} & \multicolumn{1}{c|}{M34} & \multicolumn{1}{c|}{M41} & \multicolumn{1}{c|}{M42} & \multicolumn{1}{c|}{M43} & \multicolumn{1}{c}{}                       & \multicolumn{1}{c}{}                       & \multicolumn{1}{c}{}                       & \multicolumn{1}{c|}{}                       \\ 
\hline
\multicolumn{19}{|l|}{Beta variation}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                   \\ 
\hline
\multicolumn{19}{|l|}{Beta=2}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           \\ 
\hline
3                       & 0.5                    & 0                           & 0.2                      & 0.2                      & 10                       & 1.7                      & 0.2                      & 10                       & 1.7                      & 1.7                      & 10                       & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.122,0.122,0.129}{0.9711} & \textcolor[rgb]{0.122,0.122,0.129}{0.9780} & \textcolor[rgb]{0.122,0.122,0.129}{0.9782} & \textcolor[rgb]{0.122,0.122,0.129}{0.9781}  \\ 
\hline
3                       & 0.5                    & 0                           & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & 0.9758                                     & 0.9793                                     & 0.9740                                     & 0.9789                                      \\ 
\hline
\multicolumn{19}{|l|}{Beta=0.5}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ 
\hline
3                       & 0.5                    & 0                           & 0.2                      & 0.2                      & 10                       & 1.7                      & 0.2                      & 10                       & 1.7                      & 1.7                      & 10                       & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.122,0.122,0.129}{0.9780} & \textcolor[rgb]{0.122,0.122,0.129}{0.9798} & \textcolor[rgb]{0.122,0.122,0.129}{0.9773} & \textcolor[rgb]{0.122,0.122,0.129}{0.9795}  \\ 
\hline
3                       & 0.5                    & 0                           & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.122,0.122,0.129}{0.9780} & \textcolor[rgb]{0.122,0.122,0.129}{0.9803} & \textcolor[rgb]{0.122,0.122,0.129}{0.9794} & \textcolor[rgb]{0.122,0.122,0.129}{0.9800}  \\ 
\hline
\multicolumn{19}{|l|}{Beta=0.9}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ 
\hline
3                       & 0.5                    & 0                           & 0.2                      & 0.2                      & 10                       & 1.7                      & 0.2                      & 10                       & 1.7                      & 1.7                      & 10                       & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.122,0.122,0.129}{0.9774} & \textcolor[rgb]{0.122,0.122,0.129}{0.9807} & \textcolor[rgb]{0.122,0.122,0.129}{0.9801} & \textcolor[rgb]{0.122,0.122,0.129}{0.9806}  \\ 
\hline
3                       & 0.5                    & 0                           & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.122,0.122,0.129}{0.9726} & \textcolor[rgb]{0.122,0.122,0.129}{0.9788} & \textcolor[rgb]{0.122,0.122,0.129}{0.9786} & \textcolor[rgb]{0.122,0.122,0.129}{0.9783}  \\ 
\hline
1                       & 0.5                    & 0                           & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.122,0.122,0.129}{0.9765} & \textcolor[rgb]{0.122,0.122,0.129}{0.9724} & \textcolor[rgb]{0.122,0.122,0.129}{0.9715} & \textcolor[rgb]{0.122,0.122,0.129}{0.9771}  \\ 
\hline
\multicolumn{19}{|l|}{Beta=1.1}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ 
\hline
3                       & 0.5                    & 0                           & 0.2                      & 0.2                      & 10                       & 1.7                      & 0.2                      & 10                       & 1.7                      & 1.7                      & 10                       & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.122,0.122,0.129}{0.9736} & \textcolor[rgb]{0.122,0.122,0.129}{0.9779} & \textcolor[rgb]{0.122,0.122,0.129}{0.9777} & \textcolor[rgb]{0.122,0.122,0.129}{0.9778}  \\ 
\hline
3                       & 0.5                    & 0                           & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.122,0.122,0.129}{0.9750} & \textcolor[rgb]{0.122,0.122,0.129}{0.9803} & \textcolor[rgb]{0.122,0.122,0.129}{0.9796} & \textcolor[rgb]{0.122,0.122,0.129}{0.9787}  \\ 
\hline
1                       & 0.5                    & 0                           & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & 0.9792                                     & 0.9711                                     & 0.9720                                     & 0.9801                                      \\
\hline
\end{tabular}
\end{table*}

==> table_adv_experiments3.tex <==
% \usepackage{color}


\begin{table*}
\centering
\caption{}
\label{tab:gradients3}
\resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|l|} 
\hline
\multicolumn{15}{|c|}{Parameters}                                                                                                                                                                                                                                                                                                                                                                                             & \multicolumn{4}{c|}{Accuracy}                                                                                                                                                                                                                                         & \multicolumn{1}{c|}{Index}     \\ 
\cline{1-15}
\multicolumn{2}{|c|}{KNN}                          & Warmup                               & \multicolumn{12}{c|}{Gradient}                                                                                                                                                                                                                                                                                                    & \multicolumn{4}{c|}{}                                                                                                                                                                                                                                                 & \multicolumn{1}{c|}{}          \\ 
\cline{1-2}\cline{4-19}
k                       & C                        &                                      & \multicolumn{3}{c|}{PSO-1}                                                     & \multicolumn{3}{c|}{PSO-2}                                                     & \multicolumn{3}{c|}{PSO-3}                                                     & \multicolumn{3}{c|}{PSO-4}                                                     & \multicolumn{1}{c}{PSO-1}                                       & \multicolumn{1}{c}{PSO-2}                                       & \multicolumn{1}{c}{PSO-3}                                       & PSO-4                                                           & \multicolumn{1}{c|}{}          \\ 
\cline{4-15}
                        &                          &                                      & \multicolumn{1}{c}{M12}  & \multicolumn{1}{c}{M13}  & \multicolumn{1}{c}{M14}  & \multicolumn{1}{c}{M21}  & \multicolumn{1}{c}{M23}  & \multicolumn{1}{c}{M24}  & \multicolumn{1}{c}{M31}  & \multicolumn{1}{c}{M32}  & \multicolumn{1}{c}{M34}  & \multicolumn{1}{c}{M41}  & \multicolumn{1}{c}{M42}  & M43                      & \multicolumn{1}{c}{}                                            & \multicolumn{1}{c}{}                                            & \multicolumn{1}{c}{}                                            &                                                                 &                                \\ 
\hline
3                       & 0.5                      & 0                                    & 0                        & 0                        & 0.7                      & 1                        & 1                        & 1.2                      & 1                        & 1                        & 1.2                      & 0.7                      & 0                        & 0                        & 0.9735                                                          & 0.9775                                                          & 0.9778                                                          & 0.9760                                                          & Ex19\_07                       \\ 
\hline
3                       & 0.5                      & 0                                    & 0                        & 0                        & 1.7                      & 1.7                      & 1                        & 1.7                      & 1.7                      & 1                        & 1.7                      & 1.7                      & 0                        & 0                        & 0.9741                                                          & 0.9794                                                          & 0.0793                                                          & 0.9797                                                          & Ex19\_08                       \\ 
\hline
3                       & 0.5                      & 0                                    & 0                        & 0                        & 1                        & 1                        & 1                        & 1                        & 1                        & 1                        & 1                        & 1                        & 0                        & 0                        & 0.9727                                                          & 0.9790                                                          & 0.9793                                                          & 0.9787                                                          & Ex19\_09                       \\ 
\hline
3                       & 0.5                      & 0                                    & 0                        & 0                        & 1                        & 0                        & 1                        & 0                        & 0                        & 1                        & 0                        & 1                        & 0                        & 0                        & 0.9738                                                          & 0.9782                                                          & 0.9778                                                          & 0.9784                                                          & Ex19\_10                       \\ 
\hline
3                       & 0.5                      & 0                                    & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & 0.9733                                                          & 0.9798                                                          & 0.98                                                            & 0.9795                                                          & Ex19\_11                       \\ 
\hline
3                       & 0.5                      & 0                                    & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.2                      & 1.2                      & 0.9716                                                          & 0.9786                                                          & 0.9787                                                          & 0.9782                                                          & Ex19\_12                       \\ 
\hline
3                       & 0.5                      & 0                                    & 0.2                      & 0.2                      & 0.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.2                      & 1.2                      & 0.9744                                                          & 0.9786                                                          & 0.9785                                                          & 0.9770                                                          & Ex19\_13                       \\ 
\hline
3                       & 0.5                      & 10                                   & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.2                      & 1.2                      & 0.9760                                                          & 0.9793                                                          & 0.9795                                                          & 0.9774                                                          & Ex19\_15                       \\ 
\hline
3                       & 0.5                      & 20                                   & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & 0.9771                                                          & 0.9808                                                          & 0.9806                                                          & 0.9793                                                          & Ex19\_14                       \\ 
\hline
3                       & 0.5                      & 30                                   & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & 0.9760                                                          & 0.9802                                                          & 0.9801                                                          & 0.9787                                                          & Ex19\_16                       \\ 
\hline
3                       & 1.7                      & 0                                    & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & 0.9740                                                          & 0.9797                                                          & 0.9798                                                          & 0.9801                                                          & Ex20\_04                       \\ 
\hline
3                       & 1.7                      & 10                                   & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & 0.9756                                                          & 0.9803                                                          & 0.9798                                                          & 0.9802                                                          & Ex20\_03                       \\ 
\hline
3                       & 1.7                      & 20                                   & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & 0.9743                                                          & 0.9798                                                          & 0.9801                                                          & 0.9796                                                          & Ex20\_01                       \\ 
\hline
3                       & 1.7                      & 30                                   & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & 0.9741                                                          & 0.9778                                                          & 0.9772                                                          & 0.9773                                                          & Ex20\_02                       \\ 
\hline
3                       & 1.2                      & 0                                    & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9779}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9713}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9783}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9782}                      & Ex20\_08                       \\ 
\hline
3                       & 1.2                      & 10                                   & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & 0.9758                                                          & 0.9789                                                          & 0.9789                                                          & 0.9792                                                          & Ex20\_06                       \\ 
\hline
3                       & 1.2                      & 20                                   & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & 0.9719                                                          & 0.9781                                                          & 0.9778                                                          & 0.9780                                                          & Ex20\_05                       \\ 
\hline
3                       & 1.2                      & 30                                   & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & 0.9759                                                          & 0.9791                                                          & 0.9793                                                          & 0.9781                                                          & Ex20\_07                       \\ 
\hline
3                       & 0.2                      & 0                                    & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9764}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9798}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9798}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9788}                      & \multicolumn{1}{c|}{Ex20\_09}  \\ 
\hline
3                       & 0.2                      & 10                                   & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9746}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9777}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9781}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9788}                      & \multicolumn{1}{c|}{Ex20\_10}  \\ 
\hline
3                       & 0.2                      & 20                                   & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9761}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9786}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9795}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9774}                      & \multicolumn{1}{c|}{Ex20\_11}  \\ 
\hline
3                       & 0.2                      & 30                                   & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9768}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9770}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9771}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9760}                      & \multicolumn{1}{c|}{Ex20\_12}  \\ 
\hline
3                       & 0.5                      & 0                                    & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9773}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9802}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9800}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9797}                      & \multicolumn{1}{c|}{Ex20\_13}  \\ 
\hline
3                       & 0.5                      & 10                                   & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9744}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9789}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9792}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9788}                      & \multicolumn{1}{c|}{Ex20\_14}  \\ 
\hline
3                       & 0.5                      & 20                                   & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9716}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9786}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9787}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9782}                      & \multicolumn{1}{c|}{Ex20\_15}  \\ 
\hline
3                       & 0.5                      & 30                                   & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9758}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9783}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9788}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9777}                      & \multicolumn{1}{c|}{Ex20\_16}  \\ 
\hline
3                       & 0.5                      & 0                                    & 0.2                      & 0.2                      & 10                       & 1.7                      & 0.2                      & 10                       & 1.7                      & 1.7                      & 10                       & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9774}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9814}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9814}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9816}                      & \multicolumn{1}{c|}{Ex20\_17}  \\ 
\hline
3                       & 0.5                      & 10                                   & 0.2                      & 0.2                      & 10                       & 1.7                      & 0.2                      & 10                       & 1.7                      & 1.7                      & 10                       & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9764}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9806}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9811}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9805}                      & \multicolumn{1}{c|}{Ex20\_18}  \\ 
\hline
3                       & 0.5                      & 20                                   & 0.2                      & 0.2                      & 10                       & 1.7                      & 0.2                      & 10                       & 1.7                      & 1.7                      & 10                       & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9770}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9782}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9782}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9775}                      & \multicolumn{1}{c|}{Ex20\_19}  \\ 
\hline
\multicolumn{20}{|l|}{Extend random learning rate range}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                               \\ 
\hline
\multicolumn{20}{|l|}{PSO-4's lr = [1e-5,1e1]}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ 
\hline
\multicolumn{1}{|l|}{3} & \multicolumn{1}{l|}{0.5} & \multicolumn{1}{l|}{0}               & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9669}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9696}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9714}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9629}} & Ex21\_01                       \\ 
\hline
\multicolumn{20}{|l|}{PSO-4's lr = [1e-5,1e0]}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                         \\ 
\hline
\multicolumn{1}{|l|}{3} & \multicolumn{1}{l|}{0.5} & \multicolumn{1}{l|}{20}              & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9764}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9806}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9798}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9794}} & Ex21\_02                       \\ 
\hline
\multicolumn{1}{|l|}{3} & \multicolumn{1}{l|}{0.5} & \multicolumn{1}{l|}{0}               & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9771}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9799}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9805}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9789}} & Ex21\_03                       \\ 
\hline
\multicolumn{20}{|l|}{Two random learning rates}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       \\ 
\hline
\multicolumn{20}{|l|}{PSO-1, PSO-4's lr = [1e-5, 1e-1], PSO-2's lr = 1e-3, PSO-3's lr = 1e-4}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          \\ 
\hline
\multicolumn{1}{|l|}{3} & \multicolumn{1}{l|}{0.5} & \multicolumn{1}{l|}{0}               & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9791}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9796}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9774}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9783}} & Ex22\_02                       \\ 
\hline
\multicolumn{20}{|l|}{PSO-2, PSO-4's lr = [1e-5, 1e-1], PSO-1's lr = 1e-2, PSO-3's lr = 1e-4}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          \\ 
\hline
\multicolumn{1}{|l|}{3} & \multicolumn{1}{l|}{0.5} & \multicolumn{1}{l|}{0}               & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9796}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9803}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9797}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9797}} & Ex22\_03                       \\ 
\hline
\multicolumn{20}{|l|}{PSO-3, PSO-4's lr = [1e-5, 1e-1], PSO-1's lr = 1e-2, PSO-2's lr = 1e-3}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                          \\ 
\hline
\multicolumn{1}{|l|}{3} & \multicolumn{1}{l|}{0.5} & \multicolumn{1}{l|}{0}               & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9787}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9810}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9791}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9811}} & Ex22\_01                       \\ 
\hline
\multicolumn{20}{|l|}{Three random learning rates}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                     \\ 
\hline
\multicolumn{20}{|l|}{PSO-2, PSO-3, PSO-4's lr = [1e-5,1e-1]; PSO-1's lr = 1e-2}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       \\ 
\hline
\multicolumn{1}{|l|}{3} & \multicolumn{1}{l|}{0.5} & \multicolumn{1}{l|}{0}               & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9780}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9804}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9794}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9794}} & Ex23\_01                       \\ 
\hline
\multicolumn{20}{|l|}{PSO-1, PSO-3, PSO-4's lr = [1e-5,1e-1]; PSO-2's lr = 1e-3}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       \\ 
\hline
\multicolumn{1}{|l|}{3} & \multicolumn{1}{l|}{0.5} & \multicolumn{1}{l|}{0}               & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9811}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9804}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9810}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9813}} & Ex23\_02                       \\ 
\hline
\multicolumn{20}{|l|}{PSO-1, PSO-2, PSO-4's lr = [1e-5,1e-1]; PSO-3's lr = 1e-4}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       \\ 
\hline
\multicolumn{1}{|l|}{3} & \multicolumn{1}{l|}{0.5} & \multicolumn{1}{l|}{0}               & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{1.7} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9787}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9799}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9775}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9789}} & Ex23\_03                       \\ 
\hline
\multicolumn{20}{|l|}{PSO-1, PSO-2, PSO-4's lr = [1e-5,1e-1]; PSO-3's lr = 1e-4}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       \\ 
\hline
\multicolumn{1}{|l|}{3} & \multicolumn{1}{l|}{0.5} & \multicolumn{1}{l|}{0}               & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9789}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9781}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9784}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9783}} & Ex23\_04                       \\ 
\hline
\multicolumn{20}{|l|}{PSO-1, PSO-3, PSO-4's lr = [1e-5,1e-1]; PSO-2's lr = 1e-3}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       \\ 
\hline
\multicolumn{1}{|l|}{3} & \multicolumn{1}{l|}{0.5} & \multicolumn{1}{l|}{0}               & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9812}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9806}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9816}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9809}} & Ex23\_05                       \\ 
\hline
\multicolumn{1}{|l|}{1} & \multicolumn{1}{l|}{0.5} & \multicolumn{1}{l|}{0}               & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{\textcolor[rgb]{0.129,0.129,0.129}{0.9807}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.129,0.129,0.129}{0.9796}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.129,0.129,0.129}{0.9809}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.129,0.129,0.129}{0.9798}} & Ex26\_04                       \\ 
\hline
\multicolumn{20}{|l|}{PSO-2, PSO-3, PSO-4's lr = [1e-5,1e-1]; PSO-1's lr = 1e-2}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       \\ 
\hline
\multicolumn{1}{|l|}{3} & \multicolumn{1}{l|}{0.5} & \multicolumn{1}{l|}{0}               & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9783}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9807}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9799}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9808}} & Ex23\_06                       \\ 
\hline
\multicolumn{1}{|l|}{3} & \multicolumn{1}{l|}{0.5} & \multicolumn{1}{l|}{10}              & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9802}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9793}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9794}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9792}} & Ex23\_07                       \\ 
\hline
\multicolumn{1}{|l|}{3} & \multicolumn{1}{l|}{0.5} & \multicolumn{1}{l|}{{[}0,9],[20,29]} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9765}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9800}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9780}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9786}} & Ex23\_08                       \\ 
\hline
\multicolumn{1}{|l|}{3} & \multicolumn{1}{l|}{0.5} & \multicolumn{1}{l|}{{[}0,4],[20,24]} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9796}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9799}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9794}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9801}} & Ex23\_09                       \\ 
\hline
\multicolumn{20}{|l|}{Warmup learning rates}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           \\ 
\hline
\multicolumn{20}{|l|}{PSO-1, PSO-3, PSO-4's lr = [1e-3,1e-1] in iterations [0,9] and [1e-5,1e-3] in [10,39], PSO-2's lr = 1e-3}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                        \\ 
\hline
\multicolumn{1}{|l|}{3} & \multicolumn{1}{l|}{0.5} & \multicolumn{1}{l|}{0}               & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9796}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9796}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9800}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9796}} & Ex23\_11                       \\ 
\hline
\multicolumn{20}{|l|}{PSO-1, PSO-3, PSO-4's lr = [1e-3,1e-1] in iterations [0,19] and [1e-5,1e-3] in [20,39]), PSO-2's lr = 1e-3}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\ 
\hline
\multicolumn{1}{|l|}{3} & \multicolumn{1}{l|}{0.5} & \multicolumn{1}{l|}{0}               & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9811}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9805}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9809}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9812}} & Ex23\_10                       \\ 
\hline
\multicolumn{20}{|l|}{PSO-1, PSO-3, PSO-4's lr = [1e-3,1e-1] in iterations [0,29] and [1e-5,1e-3] in [30,39], PSO-2's lr = 1e-3}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                       \\ 
\hline
\multicolumn{1}{|l|}{3} & \multicolumn{1}{l|}{0.5} & \multicolumn{1}{l|}{0}               & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9815}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9815}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9811}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.125,0.125,0.129}{0.9813}} & Ex23\_12                       \\ 
\hline
\multicolumn{1}{|l|}{1} & \multicolumn{1}{l|}{0.5} & \multicolumn{1}{l|}{0}               & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{\textcolor[rgb]{0.129,0.129,0.129}{0.9793}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.129,0.129,0.129}{0.9796}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.129,0.129,0.129}{0.9793}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.129,0.129,0.129}{0.9802}} & Ex26\_03                       \\
\hline
\multicolumn{20}{|l|}{PSO-1, PSO-3, PSO-4's lr = [1e-3,1e-1] in iterations [0,39], PSO-2's lr = 1e-3}                                        \\ 
\hline
\multicolumn{1}{|l|}{3} & \multicolumn{1}{l|}{0.5} & \multicolumn{1}{l|}{0}               & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{10}  & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{0.2} & \multicolumn{1}{l|}{\textcolor[rgb]{0.129,0.129,0.129}{0.9805}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.129,0.129,0.129}{0.9809}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.129,0.129,0.129}{0.9806}} & \multicolumn{1}{l|}{\textcolor[rgb]{0.129,0.129,0.129}{0.9789}} & Ex23\_13                       \\
\hline
\multicolumn{20}{|l|}{Formular 2}                                                                                                                                                               \\ 
\hline
\multicolumn{19}{|l|}{Ex23\_05}                                                                                                                                                                                                                                                                  & Ex27\_01                       \\ 
\hline
\multicolumn{19}{|l|}{Ex23\_12}                                                                                                                                                                                                                                                                   & Ex27\_02                       \\ 
\hline
\multicolumn{19}{|l|}{Ex23\_10}                                                                                                                                                                                                                                                                   & Ex27\_03                       \\ 
\hline
\multicolumn{19}{|l|}{Ex23\_13}                                                                                                                                                                                                                                                                   & Ex27\_04                       \\ 
\hline
\multicolumn{19}{|l|}{Ex23\_04}                                                                                                                                                                                                                                                                   & Ex27\_05                       \\ 
\hline
\multicolumn{19}{|l|}{Ex23\_06}                                                                                                                                                                                                                                                                   & Ex27\_06                       \\ 
\hline
\multicolumn{19}{|l|}{Ex23\_01}                                                                                                                                                                                                                                                                   & Ex27\_07                       \\ 
\hline
\multicolumn{19}{|l|}{Ex23\_02}                                                                                                                                                                                                                                                                   & Ex27\_08                       \\ 
\hline
\multicolumn{19}{|l|}{Ex23\_03}                                                                                                                                                                                                                                                                   & Ex27\_09                       \\
\hline
\end{tabular}
}
\end{table*}

==> table_adv_experiments4.tex <==
% \usepackage{color}


\begin{table*}
\centering
\caption{\label{tab:gradients}}
% \resizebox{\columnwidth}{!}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|l|} 
\hline
\multicolumn{15}{|c|}{Parameters}                                                                                                                                                                                                                                                                                                                                                                                             & \multicolumn{4}{c|}{Accuracy}                                                                                                                                                                                                                                         & \multicolumn{1}{c|}{Index}     \\ 
\cline{1-15}
\multicolumn{2}{|c|}{KNN}                          & Warmup                               & \multicolumn{12}{c|}{Gradient}                                                                                                                                                                                                                                                                                                    & \multicolumn{4}{c|}{}                                                                                                                                                                                                                                                 & \multicolumn{1}{c|}{}          \\ 
\cline{1-2}\cline{4-19}
k                       & C                        &                                      & \multicolumn{3}{c|}{PSO-1}                                                     & \multicolumn{3}{c|}{PSO-2}                                                     & \multicolumn{3}{c|}{PSO-3}                                                     & \multicolumn{3}{c|}{PSO-4}                                                     & \multicolumn{1}{c}{PSO-1}                                       & \multicolumn{1}{c}{PSO-2}                                       & \multicolumn{1}{c}{PSO-3}                                       & PSO-4                                                           & \multicolumn{1}{c|}{}          \\ 
\cline{4-15}
                        &                          &                                      & \multicolumn{1}{c}{M12}  & \multicolumn{1}{c}{M13}  & \multicolumn{1}{c}{M14}  & \multicolumn{1}{c}{M21}  & \multicolumn{1}{c}{M23}  & \multicolumn{1}{c}{M24}  & \multicolumn{1}{c}{M31}  & \multicolumn{1}{c}{M32}  & \multicolumn{1}{c}{M34}  & \multicolumn{1}{c}{M41}  & \multicolumn{1}{c}{M42}  & M43                      & \multicolumn{1}{c}{}                                            & \multicolumn{1}{c}{}                                            & \multicolumn{1}{c}{}                                            &                                                                 &                                \\ 
\hline
3                       & 0.5                      & 0                                    & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & 0.9733                                                          & 0.9798                                                          & 0.98                                                            & 0.9795                                                          & Ex19\_11                       \\ 
\hline
3                       & 0.5                      & 0                                    & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.2                      & 1.2                      & 0.9716                                                          & 0.9786                                                          & 0.9787                                                          & 0.9782                                                          & Ex19\_12                       \\ 
\hline
3                       & 0.5                      & 0                                    & 0.2                      & 0.2                      & 0.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.2                      & 1.2                      & 0.9744                                                          & 0.9786                                                          & 0.9785                                                          & 0.9770                                                          & Ex19\_13                       \\ 
\hline
3                       & 0.5                      & 10                                   & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.2                      & 1.2                      & 0.9760                                                          & 0.9793                                                          & 0.9795                                                          & 0.9774                                                          & Ex19\_15                       \\ 
\hline
3                       & 0.5                      & 20                                   & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & 0.9771                                                          & 0.9808                                                          & 0.9806                                                          & 0.9793                                                          & Ex19\_14                       \\ 
\hline
3                       & 0.5                      & 30                                   & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & 0.9760                                                          & 0.9802                                                          & 0.9801                                                          & 0.9787                                                          & Ex19\_16                       \\ 
\hline
3                       & 1.7                      & 0                                    & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & 0.9740                                                          & 0.9797                                                          & 0.9798                                                          & 0.9801                                                          & Ex20\_04                       \\ 
\hline
3                       & 1.7                      & 10                                   & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & 0.9756                                                          & 0.9803                                                          & 0.9798                                                          & 0.9802                                                          & Ex20\_03                       \\ 
\hline
3                       & 1.7                      & 20                                   & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & 0.9743                                                          & 0.9798                                                          & 0.9801                                                          & 0.9796                                                          & Ex20\_01                       \\ 
\hline
3                       & 1.7                      & 30                                   & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & 0.9741                                                          & 0.9778                                                          & 0.9772                                                          & 0.9773                                                          & Ex20\_02                       \\ 
\hline
3                       & 1.2                      & 0                                    & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9779}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9713}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9783}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9782}                      & Ex20\_08                       \\ 
\hline
3                       & 1.2                      & 10                                   & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & 0.9758                                                          & 0.9789                                                          & 0.9789                                                          & 0.9792                                                          & Ex20\_06                       \\ 
\hline
3                       & 1.2                      & 20                                   & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & 0.9719                                                          & 0.9781                                                          & 0.9778                                                          & 0.9780                                                          & Ex20\_05                       \\ 
\hline
3                       & 1.2                      & 30                                   & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & 0.9759                                                          & 0.9791                                                          & 0.9793                                                          & 0.9781                                                          & Ex20\_07                       \\ 
\hline
3                       & 0.2                      & 0                                    & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9764}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9798}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9798}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9788}                      & \multicolumn{1}{c|}{Ex20\_09}  \\ 
\hline
3                       & 0.2                      & 10                                   & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9746}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9777}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9781}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9788}                      & \multicolumn{1}{c|}{Ex20\_10}  \\ 
\hline
3                       & 0.2                      & 20                                   & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9761}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9786}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9795}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9774}                      & \multicolumn{1}{c|}{Ex20\_11}  \\ 
\hline
3                       & 0.2                      & 30                                   & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9768}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9770}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9771}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9760}                      & \multicolumn{1}{c|}{Ex20\_12}  \\ 
\hline
3                       & 0.5                      & 0                                    & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9773}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9802}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9800}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9797}                      & \multicolumn{1}{c|}{Ex20\_13}  \\ 
\hline
3                       & 0.5                      & 10                                   & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9744}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9789}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9792}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9788}                      & \multicolumn{1}{c|}{Ex20\_14}  \\ 
\hline
3                       & 0.5                      & 20                                   & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9716}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9786}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9787}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9782}                      & \multicolumn{1}{c|}{Ex20\_15}  \\ 
\hline
3                       & 0.5                      & 30                                   & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9758}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9783}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9788}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9777}                      & \multicolumn{1}{c|}{Ex20\_16}  \\ 
\hline
3                       & 0.5                      & 0                                    & 0.2                      & 0.2                      & 10                       & 1.7                      & 0.2                      & 10                       & 1.7                      & 1.7                      & 10                       & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9774}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9814}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9814}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9816}                      & \multicolumn{1}{c|}{Ex20\_17}  \\ 
\hline
3                       & 0.5                      & 10                                   & 0.2                      & 0.2                      & 10                       & 1.7                      & 0.2                      & 10                       & 1.7                      & 1.7                      & 10                       & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9764}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9806}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9811}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9805}                      & \multicolumn{1}{c|}{Ex20\_18}  \\ 
\hline
3                       & 0.5                      & 20                                   & 0.2                      & 0.2                      & 10                       & 1.7                      & 0.2                      & 10                       & 1.7                      & 1.7                      & 10                       & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9770}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9782}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9782}                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9775}                      & \multicolumn{1}{c|}{Ex20\_19}  \\ 
\hline
\end{tabular}
% }
\end{table*}

==> table_adv_experiments5.tex <==
% \usepackage{color}


\begin{table*}
\centering
% \resizebox{\columnwidth}{!}{
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|l|} 
\hline
\multicolumn{15}{|c|}{\begin{tabular}[c]{@{}c@{}}\\Parameters\end{tabular}}                                                                                                                                                                                                                                                                                                                                        & \multicolumn{4}{c|}{Accuracy}                                                                                                                                                     & \multicolumn{1}{c|}{Index}  \\ 
\cline{1-15}
\multicolumn{2}{|c|}{KNN}                        & \multicolumn{1}{c|}{Warmup} & \multicolumn{12}{c|}{Gradient}                                                                                                                                                                                                                                                                                                    & \multicolumn{4}{c|}{}                                                                                                                                                             & \multicolumn{1}{c|}{}       \\ 
\cline{1-2}\cline{4-19}
\multicolumn{1}{|c|}{k} & \multicolumn{1}{c|}{C} & \multicolumn{1}{c|}{}       & \multicolumn{3}{c|}{PSO-1}                                                     & \multicolumn{3}{c|}{PSO-2}                                                     & \multicolumn{3}{c|}{PSO-3}                                                     & \multicolumn{3}{c|}{PSO-4}                                                     & \multicolumn{1}{c}{PSO-1}                  & \multicolumn{1}{c}{PSO-2}                  & \multicolumn{1}{c}{PSO-3}                  & PSO-4                                      & \multicolumn{1}{c|}{}       \\ 
\cline{4-15}
\multicolumn{1}{|c|}{}  & \multicolumn{1}{c|}{}  & \multicolumn{1}{c|}{}       & \multicolumn{1}{c|}{M12} & \multicolumn{1}{c|}{M13} & \multicolumn{1}{c|}{M14} & \multicolumn{1}{c|}{M21} & \multicolumn{1}{c|}{M23} & \multicolumn{1}{c|}{M24} & \multicolumn{1}{c|}{M31} & \multicolumn{1}{c|}{M32} & \multicolumn{1}{c|}{M34} & \multicolumn{1}{c|}{M41} & \multicolumn{1}{c|}{M42} & \multicolumn{1}{c|}{M43} & \multicolumn{1}{c}{}                       & \multicolumn{1}{c}{}                       & \multicolumn{1}{c}{}                       & \multicolumn{1}{c|}{}                      &                             \\ 
\hline
\multicolumn{20}{|l|}{Beta variation}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                \\ 
\hline
\multicolumn{20}{|l|}{Beta=2}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                        \\ 
\hline
3                       & 0.5                    & 0                           & 0.2                      & 0.2                      & 10                       & 1.7                      & 0.2                      & 10                       & 1.7                      & 1.7                      & 10                       & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.122,0.122,0.129}{0.9711} & \textcolor[rgb]{0.122,0.122,0.129}{0.9780} & \textcolor[rgb]{0.122,0.122,0.129}{0.9782} & \textcolor[rgb]{0.122,0.122,0.129}{0.9781} & Ex24\_01                    \\ 
\hline
3                       & 0.5                    & 0                           & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & 0.9758                                     & 0.9793                                     & 0.9740                                     & 0.9789                                     & Ex25\_01                    \\ 
\hline
\multicolumn{20}{|l|}{Beta=0.5}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\ 
\hline
3                       & 0.5                    & 0                           & 0.2                      & 0.2                      & 10                       & 1.7                      & 0.2                      & 10                       & 1.7                      & 1.7                      & 10                       & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.122,0.122,0.129}{0.9780} & \textcolor[rgb]{0.122,0.122,0.129}{0.9798} & \textcolor[rgb]{0.122,0.122,0.129}{0.9773} & \textcolor[rgb]{0.122,0.122,0.129}{0.9795} & Ex24\_02                    \\ 
\hline
3                       & 0.5                    & 0                           & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9780} & \textcolor[rgb]{0.125,0.125,0.129}{0.9803} & \textcolor[rgb]{0.125,0.125,0.129}{0.9794} & \textcolor[rgb]{0.125,0.125,0.129}{0.9800} & Ex25\_02                    \\ 
\hline
\multicolumn{20}{|l|}{Beta=0.9}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\ 
\hline
3                       & 0.5                    & 0                           & 0.2                      & 0.2                      & 10                       & 1.7                      & 0.2                      & 10                       & 1.7                      & 1.7                      & 10                       & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.122,0.122,0.129}{0.9774} & \textcolor[rgb]{0.122,0.122,0.129}{0.9807} & \textcolor[rgb]{0.122,0.122,0.129}{0.9801} & \textcolor[rgb]{0.122,0.122,0.129}{0.9806} & Ex24\_03                    \\ 
\hline
3                       & 0.5                    & 0                           & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9726} & \textcolor[rgb]{0.125,0.125,0.129}{0.9788} & \textcolor[rgb]{0.125,0.125,0.129}{0.9786} & \textcolor[rgb]{0.125,0.125,0.129}{0.9783} & Ex25\_03                    \\ 
\hline
1                       & 0.5                    & 0                           & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9765} & \textcolor[rgb]{0.125,0.125,0.129}{0.9724} & \textcolor[rgb]{0.125,0.125,0.129}{0.9715} & \textcolor[rgb]{0.125,0.125,0.129}{0.9771} & Ex26\_02                    \\ 
\hline
\multicolumn{20}{|l|}{Beta=1.1}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                      \\ 
\hline
3                       & 0.5                    & 0                           & 0.2                      & 0.2                      & 10                       & 1.7                      & 0.2                      & 10                       & 1.7                      & 1.7                      & 10                       & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.122,0.122,0.129}{0.9736} & \textcolor[rgb]{0.122,0.122,0.129}{0.9779} & \textcolor[rgb]{0.122,0.122,0.129}{0.9777} & \textcolor[rgb]{0.122,0.122,0.129}{0.9778} & Ex24\_04                    \\ 
\hline
3                       & 0.5                    & 0                           & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & \textcolor[rgb]{0.125,0.125,0.129}{0.9750} & \textcolor[rgb]{0.125,0.125,0.129}{0.9803} & \textcolor[rgb]{0.125,0.125,0.129}{0.9796} & \textcolor[rgb]{0.125,0.125,0.129}{0.9787} & Ex25\_04                    \\ 
\hline
1                       & 0.5                    & 0                           & 0.2                      & 0.2                      & 1.7                      & 1.7                      & 0.2                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 1.7                      & 0.2                      & 0.2                      & 0.9792                                     & 0.9711                                     & 0.9720                                     & 0.9801                                     & Ex26\_01                    \\
\hline
\end{tabular}
% }
\end{table*}

==> table_comparepsoconvnets2.tex <==
\begin{table}
\centering
\caption{The comparisons between the proposed algorithm and the state-of-the-art peer competitors in terms of the classification accuracy (\%) on the Cifar-10 benchmark dataset}
\label{tab:table_comparepsoconvnets}
\begin{tabular}{|l|c|c|} 
\hline
Method                               & Accuracy (\%) & Approach                       \\ 
\hline
Tiled CNN~\cite{ngiam2010tiled}                        & 73.10         & \multirow{8}{*}{Non-PSO}            \\ 
\cline{1-2}
K-means~\cite{coates2011analysis}                        & 79.64         &            \\ 
\cline{1-2}
GA-CNN~\cite{young2015optimizing}                        & 74.59         &             \\ 
\cline{1-2}
CLR~\cite{smith2017cyclical}                        & 94.90         &             \\ 
\cline{1-2}
AmoebaNet-A~\cite{real2019regularized}                        & 96.66         &             \\ 
\cline{1-2}
ENAS~\cite{pham2018efficient}                        & 97.11         &             \\ 
\cline{1-2}
SENet~\cite{hu2018squeeze}                        & 97.88         &             \\ 
\cline{1-2}
PyramidNet AMP~\cite{zheng2021regularizing}                        & 98.02         &             \\ 
\cline{1-2}
EfficientNet-B0~\cite{tan2019efficientnet}                        & 98.10         &             \\ 
\cline{1-2}
ViT-B/16~\cite{dosovitskiy2020image}                        & 98.13         &             \\ 
\cline{1-2}
ResNet152-SAM~\cite{chen2021vision}                        & 98.20         &             \\ 
% \cline{1-2}
% GPIPE~\cite{huang2019gpipe}                        & 99.00         &             \\ 
\cline{1-2}
CaiT-M-36 U 224~\cite{touvron2021going}                        & 99.40         &             \\ 
\hline
MPSO-CNN~\cite{singh2021hybrid}                          & 89.56         & \multirow{5}{*}{PSO}            \\ 
\cline{1-2}
ModPSO-CNN~\cite{tu2021modpso}                        & 86.72         &             \\ 
\cline{1-2}
cPSO-CNN~\cite{wang2019cpso}                        & 91.35         &             \\ 
\cline{1-2}
SOBA~\cite{fielding2018evolving}                        & 95.22         &             \\ 
\cline{1-2}
EPSOCNN~\cite{wang2020particle}                           & 96.42         &            \\ 
\hline
\hline
ConvNet Baseline                       & 97.41         & Non-PSO            \\
\hline
PSO Baseline                       & 97.99         & \multirow{3}{*}{PSO}            \\
\cline{1-2}
Dynamics 1                      & 98.16         &             \\
\cline{1-2}
Dynamics 2                      & \textbf{98.31}         &             \\
\hline
\end{tabular}
\end{table}
